Automatic Generation of Socratic Subquestions for Teaching Math Word Problems

Socratic questioning is an educational method that allows students to discover answers to complex problems by asking them a series of thoughtful questions. Generation of didactically sound questions is challenging, requiring understanding of the reasoning process involved in the problem. We hypothesize that such questioning strategy can not only enhance the human performance, but also assist the math word problem (MWP) solvers. In this work, we explore the ability of large language models (LMs) in generating sequential questions for guiding math word problem-solving. We propose various guided question generation schemes based on input conditioning and reinforcement learning. On both automatic and human quality evaluations, we find that LMs constrained with desirable question properties generate superior questions and improve the overall performance of a math word problem solver. We conduct a preliminary user study to examine the potential value of such question generation models in the education domain. Results suggest that the difficulty level of problems plays an important role in determining whether questioning improves or hinders human performance. We discuss the future of using such questioning strategies in education.

==> tables/rq1-qa-subquestioning.tex <==
\begin{table}
\centering
\begin{tabular}{lr}
\hline \textbf{Variation} & \textbf{QA Accuracy} \\ \hline

\hline
\textbf{Granularity} & \\
\quad P $\oplus$ $\{q\}^{0}$ & 5.45 ($\downarrow 45\%$)\\
\quad P $\oplus$ $\{q\}^{0.25}$ &   3.94 ($\downarrow 62\%$)  \\
\quad P $\oplus$ $\{q\}^{0.5}$  &   3.35  ($\downarrow 67\%$) \\
\quad P $\oplus$ $\{q\}^{0.75}$  &   9.70  ($\downarrow 7\%$)\\
\quad P $\oplus$  $\{q\}^{1}$  & \textbf{10.46}    \\

\hline
\textbf{Order} & \\
\quad P $\oplus$ shuffle($\{q\}$)    &  8.94  ($\downarrow 14\%$)\\
\hline

\textbf{Relevance} & \\
\quad P $\oplus$ <base-ques>  &  2.57 ($\downarrow 75\%$)\\
\hline

\end{tabular}
\caption{Comparison of Math QA accuracy (in \%) for different variations of experiments with ground truth data.
$\{q\}^{k}$ represents that only $k\%$ of the ground truth sub-questions are used and selected randomly. For e.g., $\{q\}^{0.25}$ represents only $25\%$ of the sub-questions are used. $\text{shuffle}(\{q\})$ represents all sub-questions, but with shuffled order. 
Finally, \texttt{<base-ques>} are the sub-questions generated from a T5 large model without fine-tuning on our task. ($\downarrow$) represents the drop in the accuracy when compared to the Socratic questions (P $\oplus$ $\{q\}$). $\oplus$ represents the concatenation operation. GPT-2 small was used as QA model for all the above experiments.}
\label{tab:qa-subquestioning}
\end{table}


==> tables/rq2-qa-accuracy-with-reward-and-planning.tex <==
\begin{table}
\centering
\begin{tabular}{lr}
\hline \textbf{Strategy} & \textbf{QA Accuracy} \\
\hline
No planning & 6.74 \\
\quad  + rewards & 6.75 \\
\hline
Operators &  7.50  \\
\quad  + rewards &  7.52\\
\hline
Equations  &  8.49 \\
\quad + rewards &  8.50\\
\hline
\end{tabular}
\caption{Overall model variation and the influence on Math QA solver accuracy (in \%) with different planning and reward strategies. 
Here, GPT-2 small is used as the QA model.
Please note upper limit using ground truth questions is 10.46\% as shown in Table \ref{tab:qa-ques-subques}. }
\label{tab:qa-accuracy-with-reward-and-planning}
\end{table}

==> tables/rq2-qg-performance.tex <==
\begin{table}
\centering
\begin{tabular}{lccc}
\hline \textbf{Planning} & \textbf{BLEU} & \textbf{BERT F1} & \textbf{\#Q}\\ \hline
None & 51.53 & 0.783 & 0.428 \\
Operators &   54.98 & 0.788 & 0.642\\
\quad + planner & 45.05  & 0.779  & 0.346\\
Equations & \textbf{58.82} & \textbf{0.813} & \textbf{0.807} \\
\quad + planner  & 52.48   & 0.787 & 0.485 \\
\hline
\end{tabular}
\caption{\textbf{Focused questions}: QG model performance compared on the gold set of ground truth test questions with different planning strategies. Note that for the planner rows, content planning information from the ground truth data is replaced with the output from the content planner model. }
\label{table:qg-performance}
\end{table}

==> tables/rq2-qg-planning-ablation.tex <==
\begin{table}
\centering
\begin{tabular}{lccc}
\hline \textbf{Planning} & \textbf{BLEU} & \textbf{BERT F1} & \textbf{\#Q}  \\ \hline
None & 51.53 & 0.783 & 0.428 \\
Diff op, diff \# & 51.59 & 0.785 & 0.415\\
Diff op, same \#  & 54.26 & 0.786 & 0.546 \\
Operators (op) &  \textbf{54.98} & \textbf{0.788} & \textbf{0.642} \\
\hline
\end{tabular}
\caption{Manipulating the planning inputs influences the quality of generated questions and overall QG model performance. \textbf{same \#} has the same number of operators as number of reasoning steps but the types (+-/*) are shuffled, \textbf{diff \#} has both number and type of operator shuffled. }
\label{table:qg-planning-manipulation} 
\end{table}

==> tables/rq2-qg-rewards-performance.tex <==
\begin{table}
\centering
\begin{tabular}{lccc}
\hline \textbf{Strategy} & \textbf{BLEU} & \textbf{BERT F1} & \textbf{\#Q}\\ \hline
Baseline & 13.02 & 0.566 & 0.056 \\
Fine-tuned & 51.53 & 0.783 & 0.428 \\
\quad + fluency & 52.21 & 0.784 & 0.440 \\
\quad + \# of questions & 51.86 & 0.784 & 0.431 \\
\quad + QA & 52.22 &	0.783	&	0.417 \\
\quad + all weighted & 53.39 & 0.781 & 0.431  \\
Eq planning & 58.82 & 0.813 & 0.807 \\
\quad + fluency & 59.52 & \textbf{0.816} & \textbf{0.818} \\
\quad + \# of questions & \textbf{59.75} & 0.814 & 0.811 \\
\quad + QA & 59.37  & 0.813	& 0.799  \\
\quad + all weighted & 59.62 & 0.815 & 0.815  \\
\hline
\end{tabular}
\caption{\textbf{Goal-driven questions}: QG model performance compared to the gold set of ground truth questions with different rewards. }
\label{table:qg-rewards-performance}
\end{table}

==> tables/user-study-success-rate.tex <==
\begin{table}
\centering
\begin{tabular}{lcccc}
\hline \textbf{Group} & \multicolumn{2}{c}{\textbf{1st success}} & \multicolumn{2}{c}{\textbf{2nd success}} \\ %
\hline
& M & SD & M & SD \\
\hline
No-questions  &  58.4 & 23.0 & 35.8 & 32.5 \\ %
Questions  &  66.0 & 21.1  & 31.0 & 27.9\\ %
\hline
\end{tabular}
\caption{User study success rates (in \%) before after introduction of sub-questions. \textbf{1st success}  is the proportion of exercises solved correctly on the first attempt and \textbf{2nd success} is the proportion of correctly solved exercises on the second attempt (out of all incorrectly solved on the first attempt).}
\label{table:user-study-overall}
\end{table}


